Extreme heat reduces and reshapes urban mobility

Extreme heat is a problem in European countries and cities, with rising temperatures affecting ageing populations. Research on mobility during extreme heat remains limited to small samples and isolated contexts, leaving significant gaps in our understanding how entire populations adjust their day-to-day activities and how these adaptations vary across social groups. Here we use data from passive and active mobile network connections covering 13 million individuals in Spain (27% of the population) to examine extreme heat's impact on mobility at scale. We stratify by age, gender, economic class, and activity. Our findings show mobility falls by as much as 10% on hot days generally and 20% on hot afternoons specifically, when temperatures peak. Further differences emerge on hot days. Older adults cut travel to work and other activities, while those earning less are less able to avoid work; social mixing declines and spatial structure changes as activity falls in city centres. These disruptions have implications for urban economies, as curbed activity and interaction - both planned and unplanned - threaten the dynamism of cities as hubs of social and economic exchange.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
